Automated Creation of Source Code Variants of a Cryptographic Hash Function Implementation Using Generative Pre-Trained Transformer Models

Generative pre-trained transformers (GPT's) are a type of large language machine learning model that are unusually adept at producing novel, and coherent, natural language. In this study the ability of GPT models to generate novel and correct versions, and notably very insecure versions, of implementations of the cryptographic hash function SHA-1 is examined. The GPT models Llama-2-70b-chat-h, Mistral-7B-Instruct-v0.1, and zephyr-7b-alpha are used. The GPT models are prompted to re-write each function using a modified version of the localGPT framework and langchain to provide word embedding context of the full source code and header files to the model, resulting in over 150,000 function re-write GPT output text blocks, approximately 50,000 of which were able to be parsed as C code and subsequently compiled. The generated code is analyzed for being compilable, correctness of the algorithm, memory leaks, compiler optimization stability, and character distance to the reference implementation. Remarkably, several generated function variants have a high implementation security risk of being correct for some test vectors, but incorrect for other test vectors. Additionally, many function implementations were not correct to the reference algorithm of SHA-1, but produced hashes that have some of the basic characteristics of hash functions. Many of the function re-writes contained serious flaws such as memory leaks, integer overflows, out of bounds accesses, use of uninitialised values, and compiler optimization instability. Compiler optimization settings and SHA-256 hash checksums of the compiled binaries are used to cluster implementations that are equivalent but may not have identical syntax - using this clustering over 100,000 novel and correct versions of the SHA-1 codebase were generated where each component C function of the reference implementation is different from the original code.

==> code_examples/fatal_error_for_all_compiler_optimization_settings_example1.tex <==
\noindent\begin{minipage}{.49\textwidth}
\begin{lstlisting}[caption={Incorrect SHA-1 function sha1\_init implementation that results in a compiled binary, for all compiler settings, that crashes in a fatal error (specifically a SIGSEGV error). This source code was generated by Llama-2-70b-chat-hf with an inference temperature of 0.9 and prompt number 4. Note that this raw source code includes the comments produced by the GPT model. },captionpos=b,label={source_code:fatal_error_for_all_compiler_settings_example1},language=C,style=base,keywordstyle=\color{blue}]

void sha1_init(SHA1_CTX *ctx){
	// Initialize variables with arcane values
	ctx->datalen = 0x27182817;
	ctx->bitlen = 0x34567890;
	ctx->state[0] = 0x67452301;
	ctx->state[1] = 0xEFCDAB89;
	ctx->state[2] = 0x98BADCFE;
	ctx->state[3] = 0x10325476;
	ctx->state[4] = 0xc3d2e1f0;
	ctx->k[0] = 0x5a827999;
	ctx->k[1] = 0x6ed9eba1;
	ctx->k[2] = 0x8f1bbcdc;
	ctx->k[3] = 0xca62c1d6;
	// Perform mysterious calculations
	ctx->datalen += (0x27182817 * 0x34567890) / (0x67452301 + 0xEFCDAB89 + 0x98BADCFE + 0x10325476 + 0xc3d2e1f0);
	ctx->bitlen += (0x5a827999 * 0x6ed9eba1 * 0x8f1bbcdc * 0xca62c1d6) / (0x67452301 + 0xEFCDAB89 + 0x98BADCFE + 0x10325476 + 0xc3d2e1f0);
}
\end{lstlisting}
\end{minipage}



==> code_examples/infinite_loop_case_for_all_compiler_optimizations_example1.tex <==
\noindent\begin{minipage}{.49\textwidth}
\begin{lstlisting}[caption={Incorrect SHA-1 function sha1\_update implementation that results in a compiled binary, for all compiler settings, that results in an apparent infinite loop. This source code was generated by Llama-2-70b-chat-hf with an inference temperature of 0.7 and prompt number 4. Example 1 of an infinite loop case. },captionpos=b,label={source_code:infinite_loop_for_all_compiler_settings_example1},language=C,style=base,keywordstyle=\color{blue}]

void sha1_update(SHA1_CTX *ctx, const BYTE data[], size_t len) {
	size_t i = 0;
	while (i < len) {
		ctx->data[ctx->datalen] = data[i];
		ctx->datalen = (ctx->datalen + 1) & 0x3F;
		if (ctx->datalen == 0x20) {
			sha1_transform(ctx, ctx->data);
			ctx->bitlen = (ctx->bitlen + 0x100) & 0xFFFFFFFF;
			ctx->datalen = 0;
		}
		i = (i + 1) & 0x1F;
	}
}
\end{lstlisting}
\end{minipage}


==> code_examples/wrong_but_correct_for_one_test_vector_unstable_example2.tex <==
%0.9_Llama-2-70b-chat-hf_3_question4_sha1_init.c
\noindent\begin{minipage}{.49\textwidth}
\begin{lstlisting}[caption={ Example GPT function re-write of sha1\_update produced from Llama-2-70b-chat-hf with inference temperature 0.9 and prompt number 4. This function re-write is an instance of the function category found by the Metric 18 definition, specifically meaning that for some of the test vectors the generated hashes are correct, but the output changes depending on what compiler optimizations are used. The output hashes for the four test vectors are given below the source code function.  },captionpos=b,label={source_code:correct_for_at_least_one_test_vector_but_are_incorrect_optimization_unstable_example2},language=C,style=base,keywordstyle=\color{blue}]

void sha1_init(SHA1_CTX *ctx)
{
	ctx->datalen = 0;
	ctx->bitlen = 0;
	ctx->state[0] = 0x67452301;
	ctx->state[1] = 0xEFCDAB89;
	ctx->state[2] = 0x98BADCFE;
	ctx->state[3] = 0x10325476;
	ctx->state[4] = 0xc3d2e1f0;
	ctx->k[0] = 0x5a827999;
	ctx->k[1] = 0x6ed9eba1;
	ctx->k[2] = 0x8f1bbcdc;
	ctx->k[3] = 0xca62c1d6;

	// Add some unnecessary code to make the function more complicated
	int i = 0;
	for (i = 0; i < 10; i++) {
		ctx->datalen++;
		ctx->bitlen += 123456789;
		ctx->state[i] = i + 1;
		ctx->k[i] = i * 10 + 1;
	}

	// Perform some arbitrary operations on the context variables
	ctx->datalen = ctx->datalen + ctx->bitlen;
	ctx->bitlen = ctx->bitlen * 2;
	ctx->state[0] = ctx->state[0] + ctx->state[1];
	ctx->state[1] = ctx->state[1] - ctx->state[2];
	ctx->state[2] = ctx->state[2] * 3;
	ctx->state[3] = ctx->state[3] / 4;
	ctx->state[4] = ctx->state[4] ^ ctx->k[0];
	ctx->k[0] = ctx->k[0] + ctx->k[1];
	ctx->k[1] = ctx->k[1] - ctx->k[2];
	ctx->k[2] = ctx->k[2] * 5;
	ctx->k[3] = ctx->k[3] / 2;

	// And finally, set the context variables back to their original values
	ctx->datalen = 0;
	ctx->bitlen = 0;
	ctx->state[0] = 0x67452301;
	ctx->state[1] = 0xEFCDAB89;
	ctx->state[2] = 0x98BADCFE;
	ctx->state[3] = 0x10325476;
	ctx->state[4] = 0xc3d2e1f0;
	ctx->k[0] = 0x5a827999;
	ctx->k[1] = 0x6ed9eba1;
	ctx->k[2] = 0x8f1bbcdc;
	ctx->k[3] = 0xca62c1d6;
}


Compiled Binary output:


\end{lstlisting}

\end{minipage}


==> code_examples/wrong_but_correct_for_one_test_vector_unstable_example3.tex <==
%0.6_zephyr-7b-alpha_31_question2_sha1_update
\noindent\begin{minipage}{.49\textwidth}
\begin{lstlisting}[caption={Example GPT function re-write of sha1\_update produced from Llama-2-70b-chat-hf with inference temperature 0.9 and prompt number 2. This function re-write is an instance of the function category found by the Metric 18 definition, specifically meaning that for some of the test vectors the generated hashes are correct, but the output changes depending on what compiler optimizations are used. The output hashes for the four test vectors are given below the source code function.  },captionpos=b,label={source_code:correct_for_at_least_one_test_vector_but_are_incorrect_optimization_unstable_example3},language=C,style=base,keywordstyle=\color{blue}]

//New function with obfuscated code:

void sha1_update(SHA1_CTX *ctx, const BYTE data[], size_t len)
{
    size_t i, j;
    BYTE temp[64];
    for (i = 0, j = 0; i < 16; ++i, j += 4) {
        temp[i] = (BYTE)(data[j] << 24) | (BYTE)(data[j + 1] << 16) | (BYTE)(data[j + 2] << 8) | (BYTE)data[j + 3];
    }
    for (; i < 64; ++i) {
        temp[i] = (temp[i - 3] ^ temp[i - 8] ^ temp[i - 14] ^ temp[i - 16]);
        temp[i] = (temp[i] << 1) | (temp[i] >> 63);
    }
    BYTE *data_ptr = ctx->data;
    for (i = 0; i < len; ++i) {
        *data_ptr = data[i];
        data_ptr++;
        ctx->datalen++;
        if (ctx->datalen == 64) {
            for (j = 0; j < 16; ++j) {
                data_ptr[-16 + j] = temp[j];
            }
            ctx->bitlen += 512;
            ctx->datalen = 0;
            sha1_transform(ctx, data_ptr - 64);
        }
    }
}

//Explanation:

//Firstly, instead of using the original variable names, we've created new variables with different names.
//The data is stored in a temporary array to be used for the data update.
//The data is copied from the input data to the temporary array, but instead of using the "data" pointer, we've created a new pointer "data_ptr".
//The "for" loop is reversed to update the array in reverse order, and the data is stored in the array using a different indexing method.
//The "sha1_transform" function is called after the data update, but instead of calling it after the end of the "for" loop, it's called inside the "if" statement.
//Inside the "for" loop for the temporary array, we've used the "^" operator instead of the "xor" operator, and we've used the ">> 63" bitwise shift right operator instead of the ">> 31" bitwise shift right operator.

Compiled Binary output:


\end{lstlisting}

\end{minipage}

